SPEED: Streaming Partition and Parallel Acceleration for Temporal Interaction Graph Embedding

Temporal Interaction Graphs (TIGs) are widely employed to model intricate real-world systems such as financial systems and social networks. To capture the dynamism and interdependencies of nodes, existing TIG embedding models need to process edges sequentially and chronologically. However, this requirement prevents it from being processed in parallel and struggle to accommodate burgeoning data volumes to GPU. Consequently, many large-scale temporal interaction graphs are confined to CPU processing. Furthermore, a generalized GPU scaling and acceleration approach remains unavailable. To facilitate large-scale TIGs' implementation on GPUs for acceleration, we introduce a novel training approach namely Streaming Edge Partitioning and Parallel Acceleration for Temporal Interaction Graph Embedding (SPEED). The SPEED is comprised of a Streaming Edge Partitioning Component (SEP) which addresses space overhead issue by assigning fewer nodes to each GPU, and a Parallel Acceleration Component (PAC) which enables simultaneous training of different sub-graphs, addressing time overhead issue. Our method can achieve a good balance in computing resources, computing time, and downstream task performance. Empirical validation across 7 real-world datasets demonstrates the potential to expedite training speeds by a factor of up to 19.29x. Simultaneously, resource consumption of a single-GPU can be diminished by up to 69%, thus enabling the multiple GPU-based training and acceleration encompassing millions of nodes and billions of edges. Furthermore, our approach also maintains its competitiveness in downstream tasks.

==> alg_allocate.tex <==
\begin{algorithm}[!tbhp]
\label{alg:allocate}
\caption{Allocate nodes for each GPU}
    \KwIn{Pre-divided nodes lists, $n\_parts$, $\mathcal{N}$ (number of GPUs), shuffle parts or not}
    \KwOut{Allocate nodes lists to GPU}
    $parts\_multi = n\_parts / \mathcal{N}$\;
        \If{$n\_parts == \mathcal{N}$}{
        send $v_i$ nodes list to $GPU_i$ \;}
        \ElseIf{$n\_parts$ != $\mathcal{N}$ and not shuffle parts}{
        send $v_{i * parts\_multi},\cdots,v_{(i * (parts\_multi + 1))}$ node lists to $GPU_{i}$ \;}
        \ElseIf{$n\_parts$ != $\mathcal{N}$ and shuffle parts}{
        random shuffle list $\mathcal{V}$ and send $v_{i * parts\_multi},\cdots,v_{(i * (parts\_multi + 1))}$ node lists to $GPU_{i}$ \;}
\end{algorithm}

==> alg_flow.tex <==
% \SetKwComment{Comment}{/* }{ */}
\begin{algorithm}[!tbhp]
\label{alg:flow}
\caption{Accelerated Training/Validation/Testing on GPUs}
    \KwData{Original Dataset}
    % \KwOut{}
    Partition graph into different parts by Alg.\ref{alg:partitioning} and get returned list of nodes lists $\mathcal{V} = v_1,v_2,\cdots,v_c$ \;
    $parts\_multi = n\_parts / \mathcal{N}$ \;
    $parts\_multi * max(len(v_i))$ \;
    \textbf{Initialize} selected backbone model with $parts\_multi * max(len(v_i))$ nodes memory \;
    Build DDP model and send to GPUs \;
    \For{$\text{rank}=0,\cdots, \text{$\mathcal{N}$}$}{
        \For{$\text{epoch}=0,\cdots, \text{n\_epoch}$}{
            Get (combined) node list(s) \;
            Build subgraphs (full/ train/ val) and dataloaders from (combined) nodes list(s) \;
            Reset nodes memory for model \;
            Training loops Alg.\ref{alg:training} \;
            Restore nodes memory to latest memory backups \;
            \If{shared nodes exist}{sync memory between GPUs}
            Evaluate and update nodes memory state\;
            \If{shared nodes exist}{
            sync memory between GPUs \;
            save memory state for testing \;
            }
        }
    }
    \If{$\text{rank}==0$}{
    \textbf{Initialize} a model with $\sum len(v_i) $ nodes memory\;
    \If{Testing from validation end}{
    Combine all GPUs memory states into one \;
    Test\;
    }
    \ElseIf{Testing from begin}{
    Traversal train data and valid data and update nodes memory \;
    Test \;
    }
    }
    End. \
\end{algorithm}

==> tab_modules.tex <==
\begin{table}[hbt!]
\centering
\caption{Modules for different backbone models. *$(l, n)$refers to $l$ layers and $n$ neighbors}
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{cccccccc}
\toprule
                           & Mem. & \begin{tabular}[c]{@{}c@{}}Mem. \\ Updater\end{tabular} & Emb.     & \begin{tabular}[c]{@{}c@{}}Msg. \\ Agg.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Msg. \\ Func.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Msg. \\ Src.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Hit \\ Type\end{tabular} \\ \midrule
\multicolumn{1}{c|}{Jodie} & node & RNN          & time          & -         & id         & right     & none     \\
\multicolumn{1}{c|}{DyRep} & node & RNN          & id            & -         & attn       & right     & none     \\
\multicolumn{1}{c|}{TGAT}  & -    & -            & attn(2l, 20n)* & -         & -          & right     & none     \\
\multicolumn{1}{c|}{TGN}   & node & GRU          & attn(1l, 10n) & last      & id         & right     & none     \\
\multicolumn{1}{c|}{TIGE}  & node & GRU          & attn(2l, 20n) & last      & id         & left      & bin      \\ \bottomrule
\end{tabular}
}
\label{tab:modules}
\end{table}

==> tab_results.tex <==


\begin{comment}
\begin{table*}[t]
\centering
\caption{Average Precision (\%) for future edge prediction task in transductive and inductive settings. $k$ refers to the parameter $top_k$, while $k=-1$ means we do not make the restriction for $k$, which also means the algorithm degenerates to HDRF.}

\begin{tabular}{ccccccc|ccc}
\toprule
                                                                              &                                                                        &                            & Wikipeida & Reddit    & MOOC      & LastFM     & ML25m     & DGraphFin & Taobao \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Transductive}}} & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 94.87±0.7 & 94.13±0.6 & 61.54±0.8 & 65.12±5.1  & 92.22±2.1 & 74.75±1.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.68±0.9 & 93.07±0.4 & 59.69±3.2 & 58.66±1.9  & 93.99±1.4 & 78.70±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.50±0.2 & 96.69±0.3 & 61.54±0.8 & 55.97±4.3  & 93.39±1.0 & 82.16±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.34±0.0 & 98.19±0.1 & 75.32±1.1 & 83.05±0.7  & 93.09±2.4 & 82.11±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 91.12±0.3 & 90.29±1.7 & 61.87±1.2 & 67.69±0.9  & 93.70±0.5 & 74.77±0.6 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.82±1.7 & 87.14±3.8 & 60.15±1.3 & 55.77±3.8  & 87.38±4.6 & 77.86±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.90±0.1 & 92.50±1.1 & 77.34±5.4 & 62.79±6.0  & 91.32±5.5 & 82.27±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.18±0.1 & 97.81±0.2 & 84.80±1.0 & 82.20±0.7  & 92.32±2.3 & 82.41±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 94.48±1.2 & 94.07±1.5 & 63.49±0.4 & 66.89±2.8  & 93.73±0.9 & 72.69±1.9 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.29±1.3 & 93.47±1.2 & 62.76±6.6 & 53.53±2.1  & 92.74±0.7 & 77.73±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.35±0.1 & 95.84±1.2 & 81.44±2.7 & 58.98±3.7  & 94.20±0.7 & 82.08±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.22±0.1 & 98.29±0.4 & 86.80±1.9 & 82.43±0.6  & 92.73±2.8 & 82.75±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & 95.21±0.5 & 94.56±1.1 & 63.33±0.4 & 69.91±1.1  & 94.67±0.1 & 71.84±1.5 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 91.58±1.5 & 92.24±0.3 & 60.27±8.4 & 61.56±2.1  & 92.01±1.4 & 78.15±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.61±0.1 & 95.53±1.4 & 85.66±0.9 & 53.64±5.4  & 94.51±0.5 & 81.98±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.50±0.0 & 98.07±0.1 & 88.28±1.6 & 82.59±0.3  & 94.12±0.5 & 82.57±0.2 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 94.02±0.9 & 94.91±0.1 & 64.78±1.6 & 70.65±2.6  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 91.21±0.7 & 93.61±1.0 & 59.16±1.5 & 71.43±2.2  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.36±1.9 & 94.59±2.0 & 78.37±8.4 & 53.47±3.6  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.98±0.4 & 97.89±0.3 & 86.17±0.6 & 82.78±0.8  &           &           &        \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Inductive}}}    & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 93.59±0.7 & 92.86±0.2 & 61.71±0.3 & 70.43±5.6  & 91.75±2.2 & 68.76±1.6 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.40±0.5 & 93.11±0.4 & 60.05±4.1 & 69.82±1.6  & 93.68±1.3 & 64.28±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.86±0.2 & 94.84±0.5 & 76.14±1.0 & 59.32±3.8  & 93.29±0.9 & 66.11±0.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.05±0.1 & 97.40±0.3 & 79.30±3.6 & 85.32±1.1  & 92.59±2.6 & 65.98±0.4 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 88.95±0.7 & 91.39±1.2 & 60.37±1.3 & 74.58±0.7  & 93.21±0.6 & 68.91±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.33±1.4 & 90.00±2.9 & 58.68±1.5 & 63.70±6.7  & 86.72±4.9 & 64.18±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.44±0.4 & 90.71±0.3 & 77.53±3.5 & 66.94±8.4  & 91.09±5.5 & 66.51±0.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.87±0.1 & 96.86±0.3 & 84.41±1.7 & 85.27±0.9  & 92.27±2.1 & 65.41±0.2 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 92.99±1.4 & 93.18±1.7 & 61.82±0.5 & 74.53±3.3  & 93.31±1.0 & 69.21±0.5 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.12±1.4 & 93.78±0.8 & 62.82±6.1 & 61.03±3.1  & 92.43±0.7 & 64.20±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.62±0.1 & 93.95±1.7 & 81.20±3.2 & 63.79±5.9  & 93.80±0.8 & 66.82±0.4 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.91±0.1 & 97.50±0.4 & 86.30±1.8 & 84.84±1.1  & 92.31±3.0 & 65.98±0.7 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & 93.96±0.5 & 93.46±1.1 & 62.98±1.1 & 79.68±1.2  & 94.27±0.1 & 69.59±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.14±1.2 & 92.11±0.5 & 59.57±7.4 & 74.42±2.9  & 91.63±1.5 & 64.12±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.90±0.1 & 93.49±1.9 & 86.29±0.7 & 55.40±8.3  & 94.10±0.5 & 67.39±0.8 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.17±0.0 & 97.25±0.2 & 87.90±1.6 & 85.12±0.4  & 93.79±0.5 & 65.60±0.3 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 92.29±0.6 & 93.05±0.6 & 64.90±0.9 & 82.67±0.9  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.70±0.2 & 92.62±0.9 & 59.45±0.5 & 82.67±0.9  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.05±1.4 & 92.31±2.6 & 79.47±8.3 & 52.91±10.8 &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.68±0.2 & 96.96±0.2 & 86.38±0.6 & 84.44±0.6  &           &           &        \\ \bottomrule
\end{tabular}

\label{tab:performance}
\end{table*}
\end{comment}




\begin{table*}[t]
\centering
\caption{Average Precision (\%) for future edge prediction task in transductive and inductive settings. $top_k$ refers to the hyper-parameter that control the percentage of shared nodes, while $top_k=-1$ means we do not make the restriction for $top_k$, which also means the algorithm degenerates to HDRF. The best AP of different $top_k$ on different datasets and backbones are in bold.}

\begin{tabular}{ccccccc|ccc}
\toprule
                                                                              &                                                                        &                            & Wikipeida          & Reddit             & MOOC               & LastFM             & ML25m              & DGraphFin          & Taobao \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Transductive}}} & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 94.87±0.7          & 94.13±0.6          & 61.54±0.8          & 65.12±5.1          & 92.22±2.1          & 74.75±1.7          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.68±0.9          & 93.07±0.4          & 59.69±3.2          & 58.66±1.9          & \textbf{93.99±1.4} & \textbf{78.70±0.2} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.50±0.2          & \textbf{96.69±0.3} & 61.54±0.8          & 55.97±4.3          & 93.39±1.0          & 82.16±0.3          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.34±0.0          & 98.19±0.1          & 75.32±1.1          & \textbf{83.05±0.7} & 93.09±2.4          & 82.11±0.1          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 91.12±0.3          & 90.29±1.7          & 61.87±1.2          & 67.69±0.9          & 93.70±0.5          & \textbf{74.77±0.6} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.82±1.7          & 87.14±3.8          & 60.15±1.3          & 55.77±3.8          & 87.38±4.6          & 77.86±0.1          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.90±0.1          & 92.50±1.1          & 77.34±5.4          & \textbf{62.79±6.0} & 91.32±5.5          & \textbf{82.27±0.2} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.18±0.1          & 97.81±0.2          & 84.80±1.0          & 82.20±0.7          & 92.32±2.3          & 82.41±0.1          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 94.48±1.2          & 94.07±1.5          & 63.49±0.4          & 66.89±2.8          & 93.73±0.9          & 72.69±1.9          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.29±1.3          & 93.47±1.2          & \textbf{62.76±6.6} & 53.53±2.1          & 92.74±0.7          & 77.73±0.1          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.35±0.1          & 95.84±1.2          & 81.44±2.7          & 58.98±3.7          & 94.20±0.7          & 82.08±0.2          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.22±0.1          & \textbf{98.29±0.4} & 86.80±1.9          & 82.43±0.6          & 92.73±2.8          & \textbf{82.75±0.1} &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & \textbf{95.21±0.5} & 94.56±1.1          & 63.33±0.4          & 69.91±1.1          & \textbf{94.67±0.1} & 71.84±1.5          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & \textbf{91.58±1.5} & 92.24±0.3          & 60.27±8.4          & 61.56±2.1          & 92.01±1.4          & 78.15±0.1          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & \textbf{97.61±0.1} & 95.53±1.4          & \textbf{85.66±0.9} & 53.64±5.4          & \textbf{94.51±0.5} & 81.98±0.1          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & \textbf{98.50±0.0} & 98.07±0.1          & \textbf{88.28±1.6} & 82.59±0.3          & \textbf{94.12±0.5} & 82.57±0.2          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 94.02±0.9          & \textbf{94.91±0.1} & \textbf{64.78±1.6} & \textbf{70.65±2.6} &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 91.21±0.7          & \textbf{93.61±1.0} & 59.16±1.5          & \textbf{71.43±2.2} &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.36±1.9          & 94.59±2.0          & 78.37±8.4          & 53.47±3.6          &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.98±0.4          & 97.89±0.3          & 86.17±0.6          & 82.78±0.8          &                    &                    &        \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Inductive}}}    & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 93.59±0.7          & 92.86±0.2          & 61.71±0.3          & 70.43±5.6          & 91.75±2.2          & 68.76±1.6          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.40±0.5          & 93.11±0.4          & 60.05±4.1          & 69.82±1.6          & \textbf{93.68±1.3} & \textbf{64.28±0.1} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.86±0.2          & \textbf{94.84±0.5}          & 76.14±1.0          & 59.32±3.8          & 93.29±0.9          & 66.11±0.7          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.05±0.1          & 97.40±0.3 & 79.30±3.6          & \textbf{85.32±1.1} & 92.59±2.6          & \textbf{65.98±0.4} &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 88.95±0.7          & 91.39±1.2          & 60.37±1.3          & 74.58±0.7          & 93.21±0.6          & 68.91±0.1          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.33±1.4          & 90.00±2.9          & 58.68±1.5          & 63.70±6.7          & 86.72±4.9          & 64.18±0.3          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.44±0.4          & 90.71±0.3          & 77.53±3.5          & \textbf{66.94±8.4} & 91.09±5.5          & 66.51±0.7          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.87±0.1          & 96.86±0.3          & 84.41±1.7          & \textbf{85.27±0.9} & 92.27±2.1          & 65.41±0.2          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 92.99±1.4          & 93.18±1.7          & 61.82±0.5          & 74.53±3.3          & 93.31±1.0          & 69.21±0.5          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.12±1.4          & \textbf{93.78±0.8} & \textbf{62.82±6.1} & 61.03±3.1          & 92.43±0.7          & 64.20±0.3          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.62±0.1          & 93.95±1.7          & 81.20±3.2          & 63.79±5.9          & 93.80±0.8          & 66.82±0.4          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.91±0.1          & \textbf{97.50±0.4} & 86.30±1.8          & 84.84±1.1          & 92.31±3.0          & 65.98±0.7          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & \textbf{93.96±0.5} & \textbf{93.46±1.1} & 62.98±1.1          & 79.68±1.2          & \textbf{94.27±0.1} & \textbf{69.59±0.2} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & \textbf{90.14±1.2} & 92.11±0.5          & 59.57±7.4          & 74.42±2.9          & 91.63±1.5          & 64.12±0.2          &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & \textbf{96.90±0.1} & 93.49±1.9          & \textbf{86.29±0.7} & 55.40±8.3          & \textbf{94.10±0.5} & \textbf{67.39±0.8} &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & \textbf{98.17±0.0} & 97.25±0.2          & \textbf{87.90±1.6} & 85.12±0.4          & \textbf{93.79±0.5} & 65.60±0.3          &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 92.29±0.6          & 93.05±0.6          & \textbf{64.90±0.9} & \textbf{82.67±0.9} &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.70±0.2          & 92.62±0.9          & 59.45±0.5          & \textbf{82.67±0.9} &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.05±1.4          & 92.31±2.6          & 79.47±8.3          & 52.91±10.8         &                    &                    &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.68±0.2          & 96.96±0.2          & 86.38±0.6          & 84.44±0.6          &                    &                    &        \\ \bottomrule
\end{tabular}


\label{tab:performance}
\end{table*}

==> tab_results_trans.tex <==


\begin{comment}
\begin{table*}[t]
\centering
\caption{Average Precision (\%) for future edge prediction task in transductive and inductive settings. $k$ refers to the parameter $top_k$, while $k=-1$ means we do not make the restriction for $k$, which also means the algorithm degenerates to HDRF.}

\begin{tabular}{ccccccc|ccc}
\toprule
                                                                              &                                                                        &                            & Wikipeida & Reddit    & MOOC      & LastFM     & ML25m     & DGraphFin & Taobao \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Transductive}}} & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 94.87±0.7 & 94.13±0.6 & 61.54±0.8 & 65.12±5.1  & 92.22±2.1 & 74.75±1.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.68±0.9 & 93.07±0.4 & 59.69±3.2 & 58.66±1.9  & 93.99±1.4 & 78.70±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.50±0.2 & 96.69±0.3 & 61.54±0.8 & 55.97±4.3  & 93.39±1.0 & 82.16±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.34±0.0 & 98.19±0.1 & 75.32±1.1 & 83.05±0.7  & 93.09±2.4 & 82.11±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 91.12±0.3 & 90.29±1.7 & 61.87±1.2 & 67.69±0.9  & 93.70±0.5 & 74.77±0.6 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.82±1.7 & 87.14±3.8 & 60.15±1.3 & 55.77±3.8  & 87.38±4.6 & 77.86±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.90±0.1 & 92.50±1.1 & 77.34±5.4 & 62.79±6.0  & 91.32±5.5 & 82.27±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.18±0.1 & 97.81±0.2 & 84.80±1.0 & 82.20±0.7  & 92.32±2.3 & 82.41±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 94.48±1.2 & 94.07±1.5 & 63.49±0.4 & 66.89±2.8  & 93.73±0.9 & 72.69±1.9 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.29±1.3 & 93.47±1.2 & 62.76±6.6 & 53.53±2.1  & 92.74±0.7 & 77.73±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.35±0.1 & 95.84±1.2 & 81.44±2.7 & 58.98±3.7  & 94.20±0.7 & 82.08±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.22±0.1 & 98.29±0.4 & 86.80±1.9 & 82.43±0.6  & 92.73±2.8 & 82.75±0.1 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & 95.21±0.5 & 94.56±1.1 & 63.33±0.4 & 69.91±1.1  & 94.67±0.1 & 71.84±1.5 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 91.58±1.5 & 92.24±0.3 & 60.27±8.4 & 61.56±2.1  & 92.01±1.4 & 78.15±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 97.61±0.1 & 95.53±1.4 & 85.66±0.9 & 53.64±5.4  & 94.51±0.5 & 81.98±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.50±0.0 & 98.07±0.1 & 88.28±1.6 & 82.59±0.3  & 94.12±0.5 & 82.57±0.2 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 94.02±0.9 & 94.91±0.1 & 64.78±1.6 & 70.65±2.6  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 91.21±0.7 & 93.61±1.0 & 59.16±1.5 & 71.43±2.2  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.36±1.9 & 94.59±2.0 & 78.37±8.4 & 53.47±3.6  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.98±0.4 & 97.89±0.3 & 86.17±0.6 & 82.78±0.8  &           &           &        \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Inductive}}}    & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=0}}  & \multicolumn{1}{c|}{Jodie} & 93.59±0.7 & 92.86±0.2 & 61.71±0.3 & 70.43±5.6  & 91.75±2.2 & 68.76±1.6 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.40±0.5 & 93.11±0.4 & 60.05±4.1 & 69.82±1.6  & 93.68±1.3 & 64.28±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.86±0.2 & 94.84±0.5 & 76.14±1.0 & 59.32±3.8  & 93.29±0.9 & 66.11±0.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.05±0.1 & 97.40±0.3 & 79.30±3.6 & 85.32±1.1  & 92.59±2.6 & 65.98±0.4 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=1}}  & \multicolumn{1}{c|}{Jodie} & 88.95±0.7 & 91.39±1.2 & 60.37±1.3 & 74.58±0.7  & 93.21±0.6 & 68.91±0.1 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 81.33±1.4 & 90.00±2.9 & 58.68±1.5 & 63.70±6.7  & 86.72±4.9 & 64.18±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 95.44±0.4 & 90.71±0.3 & 77.53±3.5 & 66.94±8.4  & 91.09±5.5 & 66.51±0.7 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.87±0.1 & 96.86±0.3 & 84.41±1.7 & 85.27±0.9  & 92.27±2.1 & 65.41±0.2 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=5}}  & \multicolumn{1}{c|}{Jodie} & 92.99±1.4 & 93.18±1.7 & 61.82±0.5 & 74.53±3.3  & 93.31±1.0 & 69.21±0.5 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.12±1.4 & 93.78±0.8 & 62.82±6.1 & 61.03±3.1  & 92.43±0.7 & 64.20±0.3 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.62±0.1 & 93.95±1.7 & 81.20±3.2 & 63.79±5.9  & 93.80±0.8 & 66.82±0.4 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.91±0.1 & 97.50±0.4 & 86.30±1.8 & 84.84±1.1  & 92.31±3.0 & 65.98±0.7 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=10}} & \multicolumn{1}{c|}{Jodie} & 93.96±0.5 & 93.46±1.1 & 62.98±1.1 & 79.68±1.2  & 94.27±0.1 & 69.59±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 90.14±1.2 & 92.11±0.5 & 59.57±7.4 & 74.42±2.9  & 91.63±1.5 & 64.12±0.2 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.90±0.1 & 93.49±1.9 & 86.29±0.7 & 55.40±8.3  & 94.10±0.5 & 67.39±0.8 &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 98.17±0.0 & 97.25±0.2 & 87.90±1.6 & 85.12±0.4  & 93.79±0.5 & 65.60±0.3 &        \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{$top_k$=-1}} & \multicolumn{1}{c|}{Jodie} & 92.29±0.6 & 93.05±0.6 & 64.90±0.9 & 82.67±0.9  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{DyRep} & 89.70±0.2 & 92.62±0.9 & 59.45±0.5 & 82.67±0.9  &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TGN}   & 96.05±1.4 & 92.31±2.6 & 79.47±8.3 & 52.91±10.8 &           &           &        \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                  & \multicolumn{1}{c|}{TIGE}  & 97.68±0.2 & 96.96±0.2 & 86.38±0.6 & 84.44±0.6  &           &           &        \\ \bottomrule
\end{tabular}

\label{tab:performance}
\end{table*}
\end{comment}



\useunder{\uline}{\ul}{}
\begin{table*}[t]
\centering
\caption{Average Precision (\%) for future edge prediction task in transductive and inductive settings. $top_k$ refers to the hyper-parameter that control the percentage of shared nodes. When there is no restriction for $top_k$ the algorithm degenerates to HDRF. The best AP of different $top_k$ on different datasets and backbones are in bold.}

\begin{tabular}{ccccccc|ccc}
\toprule
                                                                              &                                                                       &                                 & Wikipeida          & Reddit             & MOOC               & LastFM             & ML25m              & DGraphFin          & Taobao             \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Transductive}}} & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Jodie}}} & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 94.87±0.7}    & 94.13±0.6          & 61.54±0.8          & 65.12±5.1          & 92.22±2.1          & {\ul 74.75±1.7}    & {\ul 91.43±1.1}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 91.12±0.3          & 90.29±1.7          & 61.87±1.2          & 67.69±0.9          & 93.70±0.5          & \textbf{74.77±0.6} & 91.28±0.6          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 94.48±1.2          & 94.07±1.5          & {\ul 63.49±0.4}    & 66.89±2.8          & 93.73±0.9          & 72.69±1.9          & \textbf{91.92±0.6} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{95.21±0.5} & {\ul 94.56±1.1}    & 63.33±0.4          & {\ul 69.91±1.1}    & {\ul 94.67±0.1}    & 71.84±1.5          & 90.05±1.2          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 94.02±0.9          & \textbf{94.91±0.1} & \textbf{64.78±1.6} & \textbf{70.65±2.6} & \textbf{95.01±0.1} & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{DyRep}}} & \multicolumn{1}{c|}{$top_k=0$}  & 90.68±0.9          & 93.07±0.4          & 59.69±3.2          & 58.66±1.9          & \textbf{93.99±1.4} & \textbf{78.70±0.2} & 68.71±12.2         \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 81.82±1.7          & 87.14±3.8          & 60.15±1.3          & 55.77±3.8          & 87.38±4.6          & 77.86±0.1          & {\ul 87.07±1.9}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 90.29±1.3          & {\ul 93.47±1.2}    & \textbf{62.76±6.6} & 53.53±2.1          & 92.74±0.7          & 77.73±0.1          & \textbf{89.45±0.5} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{91.58±1.5} & 92.24±0.3          & {\ul 60.27±8.4}    & {\ul 61.56±2.1}    & 92.01±1.4          & {\ul 78.15±0.1}    & 83.31±3.8          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & {\ul 91.21±0.7}    & \textbf{93.61±1.0} & 59.16±1.5          & \textbf{71.43±2.2} & {\ul 93.76±0.5}    & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{TGN}}}   & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 97.50±0.2}    & \textbf{96.69±0.3} & 61.54±0.8          & 55.97±4.3          & 93.39±1.0          & {\ul 82.16±0.3}    & {\ul 85.75±1.3}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 95.90±0.1          & 92.50±1.1          & 77.34±5.4          & \textbf{62.79±6.0} & 91.32±5.5          & \textbf{82.27±0.2} & 84.22±2.9          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 97.35±0.1          & {\ul 95.84±1.2}    & {\ul 81.44±2.7}    & {\ul 58.98±3.7}    & 94.20±0.7          & 82.08±0.2          & 81.93±8.6          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{97.61±0.1} & 95.53±1.4          & \textbf{85.66±0.9} & 53.64±5.4          & {\ul 94.51±0.5}    & 81.98±0.1          & \textbf{85.93±2.0} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 96.36±1.9          & 94.59±2.0          & 78.37±8.4          & 53.47±3.6          & \textbf{94.53±0.2} & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{TIGE}}}  & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 98.34±0.0}    & {\ul 98.19±0.1}    & 75.32±1.1          & \textbf{83.05±0.7} & {\ul 93.09±2.4}    & 82.11±0.1          & 88.03±7.4          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 98.18±0.1          & 97.81±0.2          & 84.80±1.0          & 82.20±0.7          & 92.32±2.3          & 82.41±0.1          & 88.81±3.0          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 98.22±0.1          & \textbf{98.29±0.4} & {\ul 86.80±1.9}    & 82.43±0.6          & 92.73±2.8          & \textbf{82.75±0.1} & \textbf{89.88±4.2} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{98.50±0.0} & 98.07±0.1          & \textbf{88.28±1.6} & 82.59±0.3          & \textbf{94.12±0.5} & {\ul 82.57±0.2}    & {\ul 89.04±2.9}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 97.98±0.4          & 97.89±0.3          & 86.17±0.6          & {\ul 82.78±0.8}    & 91.98±0.0          & OOM                & OOM                \\ \midrule
\multicolumn{1}{c|}{\multirow{20}{*}{\rotatebox[origin=c]{90}{Inductive}}}    & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Jodie}}} & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 93.59±0.7}    & 92.86±0.2          & 61.71±0.3          & 70.43±5.6          & 91.75±2.2          & 68.76±1.6          & 79.70±2.1          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 88.95±0.7          & 91.39±1.2          & 60.37±1.3          & 74.58±0.7          & 93.21±0.6          & 68.91±0.1          & {\ul 79.71±0.7}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 92.99±1.4          & {\ul 93.18±1.7}    & 61.82±0.5          & 74.53±3.3          & 93.31±1.0          & {\ul 69.21±0.5}    & \textbf{81.18±1.0} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{93.96±0.5} & \textbf{93.46±1.1} & {\ul 62.98±1.1}    & {\ul 79.68±1.2}    & {\ul 94.27±0.1}    & \textbf{69.59±0.2} & 78.25±2.7          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 92.29±0.6          & 93.05±0.6          & \textbf{64.90±0.9} & \textbf{82.67±0.9} & \textbf{94.66±0.1} & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{DyRep}}} & \multicolumn{1}{c|}{$top_k=0$}  & 89.40±0.5          & {\ul 93.11±0.4}    & {\ul 60.05±4.1}    & 69.82±1.6          & \textbf{93.68±1.3} & \textbf{64.28±0.1} & 59.07±6.8          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 81.33±1.4          & 90.00±2.9          & 58.68±1.5          & 63.70±6.7          & 86.72±4.9          & 64.18±0.3          & {\ul 75.25±2.8}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 89.12±1.4          & \textbf{93.78±0.8} & \textbf{62.82±6.1} & 61.03±3.1          & 92.43±0.7          & {\ul 64.20±0.3}    & \textbf{78.35±0.8} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{90.14±1.2} & 92.11±0.5          & 59.57±7.4          & {\ul 74.42±2.9}    & 91.63±1.5          & 64.12±0.2          & 71.27±4.7          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & {\ul 89.70±0.2}    & 92.62±0.9          & 59.45±0.5          & \textbf{82.67±0.9} & {\ul 93.66±0.4}    & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{TGN}}}   & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 96.86±0.2}    & \textbf{94.84±0.5} & 76.14±1.0          & 59.32±3.8          & 93.29±0.9          & 66.11±0.7          & \textbf{74.08±0.2} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 95.44±0.4          & 90.71±0.3          & 77.53±3.5          & \textbf{66.94±8.4} & 91.09±5.5          & 66.51±0.7          & 68.58±2.3          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 96.62±0.1          & {\ul 93.95±1.7}    & {\ul 81.20±3.2}    & {\ul 63.79±5.9}    & 93.80±0.8          & {\ul 66.82±0.4}    & 70.23±6.0          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{96.90±0.1} & 93.49±1.9          & \textbf{86.29±0.7} & 55.40±8.3          & \textbf{94.10±0.5} & \textbf{67.39±0.8} & {\ul 73.34±2.6}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 96.05±1.4          & 92.31±2.6          & 79.47±8.3          & 52.91±10.8         & {\ul 94.07±0.2}    & OOM                & OOM                \\ \cmidrule{2-10} 
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{TIGE}}}  & \multicolumn{1}{c|}{$top_k=0$}  & {\ul 98.05±0.1}    & {\ul 97.40±0.3}    & 79.30±3.6          & \textbf{85.32±1.1} & {\ul 92.59±2.6}    & \textbf{65.98±0.4} & {\ul 79.43±4.9}    \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=1$}  & 97.87±0.1          & 96.86±0.3          & 84.41±1.7          & {\ul 85.27±0.9}    & 92.27±2.1          & 65.41±0.2          & 76.78±4.5          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=5$}  & 97.91±0.1          & \textbf{97.50±0.4} & 86.30±1.8          & 84.84±1.1          & 92.31±3.0          & {\ul 65.98±0.7}    & \textbf{79.46±2.6} \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{$top_k=10$} & \textbf{98.17±0.0} & 97.25±0.2          & \textbf{87.90±1.6} & 85.12±0.4          & \textbf{93.79±0.5} & 65.60±0.3          & 78.37±2.3          \\
\multicolumn{1}{c|}{}                                                         & \multicolumn{1}{c|}{}                                                 & \multicolumn{1}{c|}{HDRF}       & 97.68±0.2          & 96.96±0.2          & {\ul 86.38±0.6}    & 84.44±0.6          & 91.62±0.1          & OOM                & OOM                \\ \bottomrule
\end{tabular}


\label{tab:performance}
\end{table*}
